Generalization within in silico screening

In silico screening uses predictive models to select a batch of compounds with favorable properties from a library for experimental validation. Unlike conventional learning paradigms, success in this context is measured by the performance of the predictive model on the selected subset of compounds rather than the entire set of predictions. By extending learning theory, we show that the selectivity of the selection policy can significantly impact generalization, with a higher risk of errors occurring when exclusively selecting predicted positives and when targeting rare properties. Our analysis suggests a way to mitigate these challenges. We show that generalization can be markedly enhanced when considering a model's ability to predict the fraction of desired outcomes in a batch. This is promising, as the primary aim of screening is not necessarily to pinpoint the label of each compound individually, but rather to assemble a batch enriched for desirable compounds. Our theoretical insights are empirically validated across diverse tasks, architectures, and screening scenarios, underscoring their applicability.

==> commands.tex <==
\definecolor{mygreen}{RGB}{0, 104, 55}
\definecolor{myred}{RGB}{165, 0, 38}
\definecolor{myorange}{RGB}{253, 191, 111}


\setlength{\parindent}{0em}
\setlength{\parskip}{0.5em}
\usepackage{enumitem}% http://ctan.org/pkg/enumitem
\setlist[itemize]{itemsep=2pt,topsep=0pt}
% \setlist[itemize]{noitemsep, topsep=0pt}
\renewcommand{\paragraph}[1]{\vspace{1mm}\noindent\textbf{#1}}

\newcommand{\old}[1]{}

% =================================================
\newcommand{\etal}{et al.\xspace}
\newcommand{\todo}[1]{\textcolor{orange}{\textbf{todo:}{ #1}}}
\newcommand{\andreas}[1]{\textcolor{blue}{\textbf{AL:}{ #1}}}
\newcommand{\sj}[1]{\textcolor{orange}{\textbf{SJ:}{ #1}}}
\newcommand{\tldr}[1]{\textcolor{red}{\textbf{TLDR:}{ #1}}}

\newcommand{\grad}{\b{\nabla}}
\newcommand{\relu}{\text{relu}}
\newcommand{\sigmoid}{\text{sigmoid}}
\newcommand{\diag}[1]{\text{diag}\hspace{-1px}\left(#1\right)}
\newcommand{\step}[1]{\text{step}\hspace{-1px}\left(#1\right)}
\newcommand{\rank}[1]{\text{rank}\hspace{-1px}\left(#1\right)}
\newcommand{\norm}[1]{\left\|#1\right\|}
\newcommand{\error}[1]{\text{er}\hspace{-1px}\left(#1\right)}
\newcommand{\Rbb}{\mathbb{R}}
\newcommand{\Prob}[1]{\text{P}\hspace{-1pt}\left( #1\right)}
% \newcommand{\E}[1]{\text{E}\hspace{-1pt}\left[ #1\right]}
\newcommand{\E}[2]{\mathsf{E}_{#1}\hspace{-1pt}\left[ #2\right]}
\newcommand{\Mean}[2]{\hat{\mathsf{E}}_{#1}\hspace{-1pt}\left[ #2\right]}
\newcommand{\Var}[2]{\text{Var}_{#1}\hspace{-1pt}\left[ #2\right]}
\newcommand{\indicator}[1]{\mathbf{1}\hspace{-1pt}\left[ #1\right]}
\newcommand{\from}{\leftarrow}
\DeclareMathOperator{\argmin}{argmin} 
\DeclareMathOperator{\argmax}{argmax} 
\DeclareMathOperator{\arginf}{arginf} 
\DeclareMathOperator{\argsup}{argsup} 
\DeclareMathOperator*{\avg}{avg} 
\DeclareMathOperator*{\hmean}{harm} 
\DeclareMathOperator*{\var}{var} 
\usepackage{mathtools}
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}

\renewcommand{\b}[1]{\bm{#1}}
\newcommand{\bW}{\b{W}}
\newcommand{\bA}{\b{A}}
\newcommand{\bB}{\b{B}}
\newcommand{\bD}{\b{D}}
\newcommand{\bV}{\b{V}}
\newcommand{\bR}{\b{R}}
\newcommand{\bv}{\b{v}}
\newcommand{\bI}{\b{I}}
\newcommand{\bQ}{\b{Q}}
\newcommand{\bw}{\b{w}}
\newcommand{\bk}{\b{k}}
\newcommand{\ba}{\b{a}}
\newcommand{\bb}{\b{b}}
\newcommand{\bx}{\b{x}}
\newcommand{\by}{\b{y}}
\newcommand{\bo}{\b{o}}
\newcommand{\bz}{\b{z}}
\newcommand{\bp}{\b{p}}
\newcommand{\bS}{\b{S}}
\newcommand{\bs}{\b{s}}
% \newcommand{\br}{\b{r}}
\newcommand{\bq}{\b{q}}
\newcommand{\bgamma}{\b{\gamma}}
\newcommand{\bvarphi}{\b{\varphi}}
\newcommand{\blambda}{\b{\lambda}}

% \newcommand{\cV}{\mathcal{V}}
% \newcommand{\cE}{\mathcal{E}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cZ}{\mathcal{Z}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}

\newcommand{\fE}{\mathfrak{E}}
\newcommand{\fR}{\mathfrak{R}}

\renewcommand{\bb}[1]{\mathbb{#1}}
\newcommand{\bbR}{\bb{R}}
\newcommand{\bbI}{\bb{I}}
\newcommand{\bbX}{\bb{X}}
\newcommand{\bbY}{\bb{Y}}
\newcommand{\bbZ}{\bb{Z}}

\newcommand{\risk}{r}
\newcommand{\rad}{\fR}


\usepackage{mathtools} 
\DeclarePairedDelimiter\autobracket{(}{)}
\newcommand{\br}[1]{\autobracket*{#1}}

\newtheorem{theorem}{Theorem}
\newtheorem{definition}{Definition}
\newtheorem{assumption}{Assumption}
\newtheorem{remark}{Remark}
\newtheorem{claim}{Claim}
\newtheorem{proposition}{Proposition}
\newtheorem{lemma}{Lemma}
\newtheorem{fact}{Fact}
\newtheorem{corollary}{Corollary}

